On Search Powered Navigation

Query-based searching and browsing-based navigation are the two main components of exploratory search. Search lets users dig in deep by controlling their actions to focus on and find just the information they need, whereas navigation helps them to get an overview to decide which content is most important. In this paper, we introduce the concept of "search powered navigation" and investigate the effect of empowering navigation with search functionality on information seeking behavior of users and their experience by conducting a user study on exploratory search tasks, differentiated by different types of information needs. Our main findings are as follows: First, we observe radically different search tactics. Using search, users are able to control and augment their search focus, hence they explore the data in a depth-first, bottom-up manner. Conversely, using pure navigation they tend to check different options to be able to decide on their path into the data, which corresponds to a breadth-first, top-down exploration. Second, we observe a general natural tendency to combine aspects of search and navigation, however, our experiments show that the search functionality is essential to solve exploratory search tasks that require finding documents related to a narrow domain. Third, we observe a natural need for search powered navigation: users using a system without search functionality find creative ways to mimic searching using navigation.

==> Images/Chart1-2.tex <==
\definecolor{b}{HTML}{4981CE}
\definecolor{g}{HTML}{859C27}
\definecolor{r}{HTML}{B22222}
\definecolor{o}{HTML}{FF6600}

% \makebox[\linewidth]{
% {
\begin{figure}[t]
\begin{minipage}[t]{0.47\linewidth}
    \centering
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
            % bar width= 6pt,
        },
        width= 4.7cm, % 1*\columnwidth, %\textwidth,
        height=3.2cm,
        ybar,%=0pt,
        grid=both,
        minor y tick num=2,
        ylabel={Percentage},
        xlabel={Level Jump},
        xtick=data,
        ytick = {0,10,20,30,40,50},
        xtick={1,2,3,4,5,6,7},
        xticklabels={$<-2$,-2,-1,0,1,2,$2<$},
        legend style={
            font=\fontsize{4}{5}\selectfont,
            legend image post style={xscale=0.75},
            inner sep=0pt,
            at={(0.86,-0.5)},
            legend columns=-1,
        },
        ticklabel style = {font=\fontsize{4}{5}\selectfont},
        label style={font=\fontsize{5}{6}\selectfont},
    ]
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north east lines] table[x index=0,y index=1] {\tableone};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=1] {\tableone};
    
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=2] {\tableone};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=2] {\tableone};
    
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north east lines] table[x index=0,y index=3] {\tableone};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=3] {\tableone};
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=4] {\tableone};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=4] {\tableone};
    
    \legend{\xps, ,\xps + SPN}
    
% \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
% (3.5,0.65) -- (3.5,6.5) node [black,midway,xshift=0.8cm] {\footnotesize
% $P_2$};
    \end{groupplot}
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.5,0) -- (-0.5,1.6) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{5}{6}\selectfont Broad\:-\:Topic Tasks}};
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.5,-1.6) -- (-0.5,-0.1) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{5}{6}\selectfont Focused\:-\:Topic Tasks}};
    \end{tikzpicture}
    \captionof{figure}{\label{chart:leveljump}\small Distribution of different level jumps.}
\end{minipage}
~~~~~~~~~~
\begin{minipage}[t]{0.47\linewidth} 
    \centering
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
            % bar width= 6pt,
        },
        width= 4.7cm, % 1*\columnwidth, %\textwidth,
        height=3.2cm,
        ybar,%=0pt,
        grid=both,
        minor y tick num=2,
        %ylabel={Percentage of visits},
        xlabel={Level},
        xtick=data,
        ytick = {0,10,20,30,40,50},
        xtick={1,2,3,4,5,6},
        xticklabels={1,2,3,4,5,6+},
        legend style={
            font=\fontsize{4}{5}\selectfont,
            legend image post style={xscale=0.75},
            inner sep=0pt,
            at={(0.86,-0.5)},
            legend columns=-1,
        },
        ticklabel style = {font=\fontsize{4}{5}\selectfont},
        label style={font=\fontsize{5}{6}\selectfont},
    ]
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north east lines] table[x index=0,y index=1] {\tabletwo};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=1] {\tabletwo};
    
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=2] {\tabletwo};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=2] {\tabletwo};
    
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north east lines] table[x index=0,y index=3] {\tabletwo};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=3] {\tabletwo};
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=4] {\tabletwo};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=4] {\tabletwo};
    
    \legend{\xps, ,\xps + SPN}
    
    \end{groupplot}
    % \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    % (3.5,0) -- (3.5,1.9);
    % % node [black,midway,xshift=0.8cm] {\rotatebox{270}{\fontsize{7}{8}\selectfont Broad Topic Tasks}};
    % \draw [decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    % (3.5,-2) -- (3.5,-0.1);
    % %node [black,midway,xshift=0.8cm] {\rotatebox{270}{\fontsize{7}{8}\selectfont Focused Topic Tasks}};
    \end{tikzpicture}
    
   \captionof{figure}{\label{chart:level}\small Distribution of level visits.}
\end{minipage}
\end{figure}
% }

==> Images/Chart3-Table2.tex <==
\definecolor{b}{HTML}{4981CE}
\definecolor{g}{HTML}{859C27}
\definecolor{r}{HTML}{B22222}
\definecolor{o}{HTML}{FF6600}
\newcommand{\multilinecell}[2][c]{%
\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}
}
\begin{figure}[t]
\makebox[\linewidth]{
%\begin{minipage}[t]{0.56\linewidth}
\begin{minipage}[t]{1\linewidth}
\centering
\vspace{0pt}
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
            % bar width= 6pt,
        },
        width= 6.5cm, % 1*\columnwidth, %\textwidth,
        height=4cm,
        ybar,%=0pt,
        % bar width= 6pt,
        grid=both,
        minor y tick num=2,
        ylabel={Percentage},
        xlabel={Edge Rank},
        xtick=data,
        xtick={1,2,3,4,5,6},
        xticklabels={1,2,3,4,5,6+},
        legend style={at={(-0.1,0.96),font=\fontsize{5}{6}}
          legend columns=-1
          },
        ticklabel style = {font=\fontsize{6}{7}\selectfont},
        label style={font=\fontsize{7}{8}\selectfont},
    ]
    \nextgroupplot[ytick = {0,10,20,30,40},]
    \addplot [thick, b ,line join=round,smooth, fill=b, draw=none, pattern color=b, pattern = crosshatch] table[x index=0,y index=2] {\tablethree} \closedcycle;

    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=2] {\tablethree};
    
    \addplot [fill= r, draw= r, pattern color = r] table[x index=0,y index=1] {\tablethree};
    \legend{System Score, ,User Selection}
    
    \nextgroupplot[ytick = {0,20,40,60,80},]
    \addplot [thick, b ,line join=round,smooth, fill=b, draw=none, pattern color=b, pattern = crosshatch] table[x index=0,y index=4] {\tablethree} \closedcycle;
    
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=4] {\tablethree};
    
    \addplot [fill= r, draw= r, pattern color = r] table[x index=0,y index=3] {\tablethree};
    
    \legend{System Score, ,User Selection}
    
    \end{groupplot}
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.7,0) -- (-0.7,2.4) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Broad\:-\:Topic Tasks}};
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.7,-2.4) -- (-0.7,-0.1) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Focused Topic\:-\:Tasks}};
    %\vspace{-10pt}
    \end{tikzpicture}
    \caption{\label{chart:rank}Percentage of the selected edges on different ranks versus the distribution of scores assigned by the system to edges over different ranks.}
\end{minipage}
~~~~
%\begin{minipage}[t]{0.4\linewidth} 
%\centering
%\vspace{0pt}
%\captionof{table}{\label{tbl:tbl2} Statistics from search sessions using the system with SPN grouped by gender. The given numbers are per-session statistics, averaged over all search sessions. The difference between numbers in the same column is statistically significant (two-tailed t-test, p-value $<$ 0.05).}
%\vspace{3pt}
%\makebox[\linewidth][c]{
%\begin{adjustbox}{max width= \textwidth} %\columnwidth}
%{\renewcommand{\arraystretch}{1.3} 
%\begin{tabular} 
%{l c c c c c c c c c}
%{@{}l@{~~~}c@{~~}c@{}}
%\toprule
%\fontsize{6}{7}\selectfont
%\textbf{Gender} & 
%\multilinecell{\textbf{avg. num. of} \\ \textbf{query} \\ \textbf{submissions}} &
%\multilinecell{\textbf{avg. num. of} \\ \textbf{expansion before} \\ \textbf{the first search}} \\
%\midrule
%\textbf{Female} & 8.1 &  6.3
%\\
%\midrule
%\textbf{Male} & 20.6 & 2.7 
%\\
%\bottomrule 
%\end{tabular}
%}
%\end{adjustbox}
%}
%\end{minipage}
}
\end{figure}
% }

==> Images/resultFigs.tex <==
\definecolor{b}{HTML}{4981CE}
\definecolor{g}{HTML}{859C27}
\definecolor{r}{HTML}{B22222}
\definecolor{o}{HTML}{FF6600}


\begin{figure*}[t]
% \makebox[\linewidth][c]{
% \centering
\centerline{
\begin{minipage}[b]{0.6\textwidth}
\captionsetup[subfigure]{margin={1.5cm,-0.1cm}}
\begin{subfigure}{0.49\textwidth}
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
        },
        width= 5.7cm, % 1*\columnwidth, %\textwidth,
        height=3cm,
        ybar,%=0pt,
        grid=both,
        minor y tick num=0.5,
        ylabel={Percentage},
        xlabel={Level Jump},
        xtick=data,
        ytick = {0,10,20,30,40,50},
        xtick={1,2,3,4,5,6,7},
        xticklabels={$<$-2,-2,-1,0,1,2,2$<$},
        legend style={
            font=\fontsize{6}{7}\selectfont,
            legend image post style={xscale=0.75},
            inner sep=0pt,
            at={(0.86,-0.5)},
            legend columns=-1,
        },
        ticklabel style = {font=\fontsize{6}{7}\selectfont},
        label style={font=\fontsize{7}{8}\selectfont},
    ]
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north west lines] table[x index=0,y index=1] {\tableone};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=1] {\tableone};
%    
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=2] {\tableone};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=2] {\tableone};
%    
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north west lines] table[x index=0,y index=3] {\tableone};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=3] {\tableone};
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=4] {\tableone};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=4] {\tableone};
%
    \end{groupplot}
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.55,0) -- (-0.55,1.4) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Broad\:-\:Topic}};
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.55,-1.4) -- (-0.55,0) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Focused\:-\:Topic}};
    \end{tikzpicture}
    \caption{\label{chart:leveljump}\small Distribution of level jumps.}
\end{subfigure}
%
\hspace{-30pt}
%\hfill
\begin{subfigure}{0.49\textwidth}
    \centering
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
            % bar width= 6pt,
        },
        width= 5.7cm, % 1*\columnwidth, %\textwidth,
        height=3cm,
        ybar,%=0pt,
        grid=both,
        minor y tick num=1,
        %ylabel={Percentage of visits},
        xlabel={Level},
        xtick=data,
        ytick = {0,10,20,30,40,50},
        xtick={1,2,3,4,5,6},
        xticklabels={1,2,3,4,5,6+},
        legend style={
            font=\fontsize{6}{7}\selectfont,
            legend image post style={xscale=0.75},
            %inner sep=0pt,
            at={(0.3,-0.3)},
            legend columns=-1,
        },
        ticklabel style = {font=\fontsize{6}{7}\selectfont},
        label style={font=\fontsize{7}{8}\selectfont},
    ]
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north west lines] table[x index=0,y index=1] {\tabletwo};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=1] {\tabletwo};
%    
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=2] {\tabletwo};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=2] {\tabletwo};
%    
    \nextgroupplot
    \addplot [fill=b, draw=b, pattern color = b, pattern = north west lines] table[x index=0,y index=3] {\tabletwo};
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=3] {\tabletwo};
    \addplot [fill=r, draw=r, pattern color = r, pattern = north east lines] table[x index=0,y index=4] {\tabletwo};
    \addplot [thick,r ,line join=round,smooth] table[x index=0,y index=4] {\tabletwo};
%    
    \legend{\xps, ,\xps + SPN}
%    
    \end{groupplot}
    \end{tikzpicture}
  \caption{\label{chart:level}\small Distribution of level visits.}
\end{subfigure}
\vspace{-10pt}
\caption{Distribution of level jumps and visits for focused and broad topics.}
\end{minipage}
%
\hspace{\stretch{2}}
%
\begin{minipage}[b]{0.38\textwidth}
\centering
    \begin{tikzpicture}
    \begin{groupplot}[
        /pgf/bar width=6pt,
        group style={
            group name=Mosi Plot,
            group size=1 by 2,
            xlabels at=edge bottom,
            xticklabels at=edge bottom,
            vertical sep=0pt,
        },
        width= 5.7cm, % 1*\columnwidth, %\textwidth,
        height=3cm,
        ybar,
        grid=both,
        minor y tick num=0.5,
        ylabel={Percentage},
        xlabel={Edge Rank},
        xtick=data,
        xtick={1,2,3,4,5,6},
        xticklabels={1,2,3,4,5,6+},
        legend style={
            at={(0.8,-0.6),font=\fontsize{6}{7}},
            legend columns=-1
        },
        ticklabel style = {font=\fontsize{6}{7}\selectfont},
        label style={font=\fontsize{7}{8}\selectfont},
    ]
    \nextgroupplot[ytick = {0,10,20,30,40},]
    \addplot [thick, b ,line join=round,smooth, fill=b, draw=none, pattern color=b, pattern = crosshatch] table[x index=0,y index=2] {\tablethree} \closedcycle;
%
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=2] {\tablethree};
%    
    \addplot [fill= r, draw= r, pattern color = r] table[x index=0,y index=1] {\tablethree};
%    
    \nextgroupplot[ytick = {0,20,40,60,80},]
    \addplot [thick, b ,line join=round,smooth, fill=b, draw=none, pattern color=b, pattern = crosshatch] table[x index=0,y index=4] {\tablethree} \closedcycle;
%    
    \addplot [thick, b ,line join=round,smooth] table[x index=0,y index=4] {\tablethree};
%    
    \addplot [fill= r, draw= r, pattern color = r] table[x index=0,y index=3] {\tablethree};
%    
    \legend{System Score, ,User Selection}
%    
    \end{groupplot}
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.55,0) --  (-0.55,1.4) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Broad\:-\:Topic}};
    \draw [decorate,decoration={brace,amplitude=10pt},xshift=-4pt,yshift=0pt]
    (-0.55,-1.4) -- (-0.55,0) node [black,midway,xshift=-0.6cm] 
    {\rotatebox{90}{\fontsize{6}{7}\selectfont Focused\:-\:Topic}};
    \end{tikzpicture}
    \vspace{-10pt}
    \captionof{figure}{\label{chart:rank}\small{Percentage of selected edges on different ranks versus distribution of scores assigned to edges.}}
\end{minipage}
}
\vspace{-15pt}
\end{figure*}

==> Table3.tex <==
%\begin{table}[t]
\begin{table}%{r}{5.5cm}
\captionof{table}{\label{tbl:tbl3}Average rating (on a 10-point scale) given by two assessors to the generated summaries and set of relevant speeches as the outcome of the search sessions.}
%\todo{Are there any satistically significant differences in the table?}
\vspace{4pt}
\makebox[\linewidth][c]{
\begin{adjustbox}{max width=0.45\textwidth} %\columnwidth}
{\renewcommand{\arraystretch}{1} 
\begin{tabular} 
%{l c c c c c c c c c}
{@{}l@{~~~}c@{~~}c@{}}
\toprule
%\fontsize{6}{7}\selectfont
\textbf{\multilinecell{System Type / \\ Task Type}} & \textbf{\xps} & \textbf{\xps+SPN} \\
\midrule
\textbf{Broad\:-\:Topic} & \multilinecell{5.12 \\ (SD=1.71)} &  \multilinecell{7.78 \\ (SD=2.16)}
\\
\midrule
\textbf{Focused\:-\:Topic} & \multilinecell{3.44 \\ (SD=2.65)} &  \multilinecell{4.62 \\ (SD=2.40)}
\\
\bottomrule 
\end{tabular}
}
\end{adjustbox}
}
%\end{table}
\end{table}












% \begin{table}[tbp]
% \centering
% \caption{\label{tbl:tbl2} Statistics from search sessions using the system with \spn grouped by participants gender in our users study. The given numbers are per-session statistics, averaged over all search sessions. The difference between numbers marked by $^\blacktriangleup$ or $^\blacktriangledown$ with other numbers in the same column is statistically significant.}
% \vspace{3pt}
% \makebox[\linewidth][c]{
% \begin{adjustbox}{max width= 0.5\textwidth} %\columnwidth}
% {\renewcommand{\arraystretch}{1.35} 
% \begin{tabular} 
% %{l c c c c c c c c c}
% {@{}c@{~~}l@{~~~}c@{~~}c@{}}
% \toprule
% %\fontsize{6}{7}\selectfont
% \textbf{System} & \textbf{Gender} & 
% \multilinecell{\textbf{avg. num. of query} \\ \textbf{submissions}} &
% \multilinecell{\textbf{avg. num. of expansion} \\ \textbf{before the first search}} \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\multilinecell{Broad \\ Topic}}} & Female & & 
% \\
% \cmidrule(lr){2-4}
% & Male & & \\
% \midrule
% \multirow{2}{*}{\rotatebox{90}{\multilinecell{Focused \\ Topic}}} & Female &  &  \\
% \cmidrule(lr){2-4}
% & Male &  &  \\
% \bottomrule 
% \end{tabular}
% }
% \end{adjustbox}
% }
% %\vspace{-10pt}
% \end{table}
